SolidGen: An Autoregressive Model for Direct B-rep Synthesis

The Boundary representation (B-rep) format is the de-facto shape representation in computer-aided design (CAD) to model solid and sheet objects. Recent approaches to generating CAD models have focused on learning sketch-and-extrude modeling sequences that are executed by a solid modeling kernel in postprocess to recover a B-rep. In this paper we present a new approach that enables learning from and synthesizing B-reps without the need for supervision through CAD modeling sequence data. Our method SolidGen, is an autoregressive neural network that models the B-rep directly by predicting the vertices, edges, and faces using Transformer-based and pointer neural networks. Key to achieving this is our Indexed Boundary Representation that references B-rep vertices, edges and faces in a well-defined hierarchy to capture the geometric and topological relations suitable for use with machine learning. SolidGen can be easily conditioned on contexts e.g., class labels, images, and voxels thanks to its probabilistic modeling of the B-rep distribution. We demonstrate qualitatively, quantitatively, and through perceptual evaluation by human subjects that SolidGen can produce high quality, realistic CAD models.

==> SolidGen TMLR arXiv/0-abstract.tex <==
The Boundary representation (B-rep) format  is the de-facto shape representation in computer-aided design (CAD) to model solid and sheet objects. Recent approaches to generating CAD models have focused on learning sketch-and-extrude modeling sequences that are executed by a solid modeling kernel in postprocess to recover a B-rep. In this paper we present a new approach that enables learning from and synthesizing B-reps without the need for supervision through CAD modeling sequence data. Our method SolidGen, is an autoregressive neural network that models the B-rep directly by predicting the vertices, edges, and faces using Transformer-based and pointer neural networks. Key to achieving this is our Indexed Boundary Representation that references B-rep vertices, edges and faces in a well-defined hierarchy to capture the geometric and topological relations suitable for use with machine learning. SolidGen can be easily conditioned on contexts e.g., class labels, images, and voxels thanks to its probabilistic modeling of the B-rep distribution. We demonstrate qualitatively, quantitatively, and through perceptual evaluation by human subjects that SolidGen can produce high quality, realistic CAD models.

==> SolidGen TMLR arXiv/1-introduction.tex <==
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.99\textwidth]{figures/Teaser.jpg}
    \caption{SolidGen generates B-reps incrementally by building vertices, edges, and faces one at a time. Here we show snapshots from the edge (columns 1--2) and face generation (columns 3--8) for two data samples.}
    \label{fig:teaser}
\end{figure}
\section{Introduction}
Almost every manufactured object in the world starts life as a computer-aided design (CAD) model.
The Boundary representation format (B-rep) is the de-facto standard used in CAD to represent solid and sheet objects as a collection of trimmed parametric surfaces connected with well-structured topology~\citep{weiler1986}.
The ability to generate B-reps automatically, driven by some context, is an enabling technology for design exploration and is critical to solving a range of problems in CAD such as reverse engineering from noisy 3D scan data, inpainting holes in solid models plausibly, and design synthesis from images or drawings.

Recent approaches to the generation of CAD models have focused on generating sequences of CAD modeling operations \citep{willis2020fusion,xu2021zone,wu2021deepcad,xu2022skexgen,lambourne2022}, rather than the underlying 3D geometry and topology in the B-rep format. These methods produce a sequence of sketch and extrude modeling operations using a neural network and the B-rep is recovered in postprocess with a solid modeling kernel that executes the operations.
Although this approach generates an editable CAD model, it is currently limited to the sketch and extrude modeling operations and cannot be easily extended to support other operations or build sheet bodies.
In particular, fillets and chamfers, which are widely used in CAD for structural performance and ease of manufacture, are challenging as they operate on B-rep edges which are not available until the predicted solid has been built.
Furthermore, sketch-and-extrude workflows operate with 2D planar curves, hence extensions to freeform modeling are not trivial.

There are several advantages to pursuing an approach that directly synthesizes the B-rep. Firstly, significantly more CAD data exists without a stored sequence of CAD modeling operations. Files created via direct modeling or exported to common B-rep file formats do not retain a history of CAD modeling operations. In the public domain, CAD model datasets with CAD modeling operations~\citep{willis2020fusion,wu2021deepcad} are smaller ($\sim$190K models) than those without~\citep{koch2019abc} (1M models).
Secondly, support for freeform curves and surfaces like B\'ezier and non-uniform rational B-splines, or advanced topological structures like T-splines or Catmull-Clark subdivision meshes can be provided with the ability to generate B-reps directly, as they share geometric and topological similarities.
Finally, there are several problems in CAD that can only be solved with a direct B-rep synthesis approach. Examples include hole-filling for repairing solids which have poorly trimmed or missing faces due to data exchange~\citep{butlin1996cad,Assadi2003CADMR}, patching up geometry in regions of a model where error-prone operations, such as offsetting, fail~\citep{bodily2014computational} and the
creation of parting surfaces and shut-outs in molding workflows~\citep{bhargava1991automated,Serrar1995}.
Although heuristic algorithms exist for such applications, a learning-based method has the potential to incorporate external context and respect aesthetic aspects of the CAD model.

We make the following contributions in this paper:
\begin{itemize}[leftmargin=*,topsep=1pt]
	\item We propose SolidGen, a novel generative model based on Transformers and two-level pointer networks for the direct synthesis of B-reps (\autoref{fig:teaser}) without  supervision from a sequence of CAD modeling operations. To the best of our knowledge, SolidGen is the first generative model that can synthesize B-reps directly.
	\item We propose a new representation, the indexed boundary representation, that can represent B-reps as numeric arrays suitable for use with machine learning, while still allowing the geometry and topology of B-reps to be completely recovered.
    \item We show the quantitative and qualitative performance of SolidGen for unconditional generation and perform a perceptual study showing SolidGen produces more realistic results than the state-of-the-art.
    \item We demonstrate how controllable generation of B-reps can be achieved by conditioning with class labels, images, and voxels when available. 
\end{itemize}


==> SolidGen TMLR arXiv/2-related-work.tex <==
\section{Related Work}
Since the proliferation of the B-rep format~\citep{lee2001partialentity,slyadnev2020role,weiler1986} in the 1980s, several research areas have been explored. 

\myparagraph{Learning from B-reps.}
The ability to represent B-rep data as a graph~\citep{ansaldi1985geometric} has inspired recent approaches using graph neural networks for classification and segmentation problems~\citep{cao2020gnn,jayaraman2021uvnet}. B-rep topology can also be used for custom convolutions~\citep{lambourne2021brepnet} or hierarchical graph structures~\citep{jones2021automate}. Rather than an \textit{encoder}, our work focuses on a \textit{decoder} to synthesize B-rep data directly.

\myparagraph{Constructive Solid Geometry (CSG).}
In CSG, 3D shapes are formed by combining primitives (e.g. cuboids, spheres) with Boolean operations (e.g. union, subtraction) into a CSG tree. By parsing the tree with an appropriate geometry kernel, a B-rep can be obtained. CSG approaches have been used to reconstruct `shape programs' in combination with techniques from the program synthesis literature, both with neural guidance~\citep{sharma2018csgnet,ellis2019write,tian2019learning,kania2020ucsg} and without~\citep{du2018inversecsg,nandi2017programming,nandi2018functional}. By contrast, our work applies to multiple tasks beyond reconstruction.

\myparagraph{Sequential CAD Generation.}
Another line of research leverages the supervision available from modeling operations stored in parametric CAD files to directly predict sequences of CAD modeling operations. The result is editable CAD files in the form of 2D engineering sketches~\citep{willis2021engineering,para2021sketchgen,ganin2021computer,seff2021vitruvion} or 3D CAD models generated from a B-rep~\citep{willis2020fusion,xu2021zone} or point cloud~\citep{Point2CylUy} target, interactive system~\citep{li2020sketch2cad}, or generative model~\citep{wu2021deepcad,xu2022skexgen}. 
Although sequential CAD generation approaches have made significant progress, an outstanding challenge is how to extend these techniques to other modeling operations beyond sketch and extrude. Common modeling operations, such as fillet and chamfer, are challenging as they operate on B-rep edges which are not part of the representation available to the network, but rather generated as a post-process. An alternate approach might be to use reinforcement learning with a CAD kernel integrated into the environment, similar to \cite{lin2020modeling}, at the expense of extended training times due to the sparse reward space and slow CAD kernel execution times.
Instead, we focus our efforts on direct synthesis of the B-rep data structure which cannot be achieved by predicting a sequence of CAD modeling operations.

\myparagraph{Direct B-rep Generation.}
Direct B-rep generation involves the synthesis of the underlying parametric curves/surfaces and the topology that connects them to form a solid model. Several learning-based approaches have made progress with the generation of parametric curves~\citep{wang2020pie} and surfaces~\citep{sharma2020parsenet}. Yet to be addressed is a generative model for the creation of topology that joins parametric curves and surfaces together to form solid models, rather than relying on pre-defined topological templates \citep{smirnov2021patches}.
PolyGen~\citep{nash2020polygen} is a promising approach to joint geometry and topology synthesis where sequences of $n$-gon mesh vertices and faces are predicted using Transformers~\citep{vaswani2017transformer}. A key insight of this work is the use of pointer networks~\citep{vinyals2015pointer} to reference previously predicted primitives and form the underlying shape topology. Our work draws inspiration from the use of pointer networks to develop a novel representation and method for the challenging task of direct B-rep generation.
\cite{wang2022neuralface} concurrently applied a pointer network to identify planar and cylindrical faces given the 2D projection of edges. Our method is more general and synthesizes the entire B-rep while supporting all prismatic surfaces in a generative modeling framework.
A similar representation to ours was proposed in a concurrent work \citep{guo2022complexgen}, where the objective was to reverse engineer B-reps from point clouds. Using a neural network to predict the rough B-rep geometry and topology, a combinatorial optimization was applied to refine the solution. By contrast, our method is an autoregressive generative model with support for more input modalities such as image and class in addition to point clouds, and does not require an expensive optimization step to build plausible B-reps.

==> SolidGen TMLR arXiv/3-representation.tex <==
\section{Representation}

\begin{figure*}
    \centering
{\includegraphics[width=0.9\textwidth]{figures/BRepEntityTypesv01.pdf}}
    \caption{The Boundary Representation data structure consists of vertices, edges formed by curve primitives (left) and faces formed by surface primitives (right). Loops of oriented edges---wires, are used to delimit the surfaces into visible and hidden regions.}
    \label{fig:brep_entities}
\end{figure*}


\myparagraph{Boundary Representation.}
B-reps are a kind of generalized mesh structure in which many of the restrictions of triangle meshes have been removed (\autoref{fig:brep_entities}). In place of planar triangular facets, B-reps allow \textit{faces} built from planes, cylinders, cones, spheres, toroidal surfaces or B-splines surfaces. The \textit{edges} at the boundary of faces can be lines, arcs, circles or B-spline curves.   Unlike meshes, B-rep faces can have internal holes, hence closed loops of edges are organized into oriented \textit{wires} to delimit the surfaces.
The curves defining the edges can be viewed as functions from an interval in the 1D u-parameter domain into 3D, while the surfaces can be viewed as functions from a 2D box in the uv-parameter domain to 3D. The wires defining a face's boundaries can be projected onto its surface's 2D parameter domain, forming closed loops. Outer loops in uv-space are oriented anti-clockwise, while inner loops are in clockwise direction. This allows uv-points to be classified as visible or hidden and facilitates meshing~\citep{chew1987delaunay,Rockwood1989}
\footnote{For periodic surfaces (cylinders, cones, spheres and tori), which have parameter domains ``topologically glued" from 0 to 2$\pi$  in one or both dimensions, the surface must first be subdivided into patches homeomorphic to the disk.}.
The B-rep data structure stores many references among entities (typically using pointers) allowing efficient constant-time querying of adjacency information~\citep{lee2001partialentity}.

\myparagraph{Indexed Boundary Representation.}
We now derive an indexed representation of the B-rep (\autoref{fig:representation}, right) that can be represented as numeric arrays suitable for use with machine learning.
Importantly, this representation can be inverted back into a B-rep exactly.
We currently restrict the representation to elementary curves (lines and arcs) and surfaces (planes, cylinders, cones, spheres and tori).
We do not support B-splines and conic sections that are uncommon in mechanical CAD~\citep{willis2020fusion,koch2019abc}.
Without loss of generality, we assume that closed faces (cylinders, cones, etc.) in the B-rep are all split on the seams to simplify downstream processing, for e.g., a closed cylinder with a seam is split into two four sided half-cylinders.
The indexed B-rep is analogous to the indexed list data structure used to represent polygonal meshes, e.g. the Wavefront OBJ file format~\citep{wavefrontOBJ}.
The indexed list data structure can be represented numerically using two lists of numbers, and has been successfully used for generative modeling of meshes~\citep{nash2020polygen} and engineering sketches~\citep{willis2021engineering}.
Just as a polygonal mesh can be represented using a topological data structure like winged edge \citep{Baumgart1972}, or a simple data structure like the indexed list, we show that B-reps can be converted into an indexed format.
However, while a polygonal mesh is restricted to straight line edges and planar faces, B-reps are more general with support for curved edges and faces,  making our problem more challenging.
We address this challenge by explicitly representing only the bare minimum geometric and topological information in our indexed format, and designing a rule-based algorithm leveraging solid modeling kernels to infer and build the rest of the information.
The indexed B-rep $\brep$ is comprised of three lists $\{\vertex, \edge, \face\}$:
\textit{Vertices $\vertex$} contain a list of 3D point coordinates corresponding to each B-rep vertex and the arc midpoints.
\textit{Edges $\edge$} are represented as hyperedges~\citep{willis2021engineering} where each hyperedge is a list of indices into $\vertex$.
A hyperedge connects two or more vertices to define the edge geometry. The  curve type is defined by the cardinality of the hyperedge: line (2), arc (3).
\textit{Faces $\face$} are defined as the set of edges bounding a surface. Each face contains a list of indices into $\edge$.
By indexing from \textit{Faces}, to \textit{Edges}, to \textit{Vertices}, our representation is well suited for use with pointer networks~\citep{vinyals2015pointer}. Parametric surfaces that define the geometry of the face, and wires that trim the surfaces are left out of our representation and recovered in postprocess, as described next.

\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/SolidGenRepresentationv04.pdf}
    \put(-262pt,12pt){{$\scriptstyle\vertex$}}
    \put(-163pt,12pt){{$\scriptstyle\edge$}}
    \put(-35.2pt,12pt){{$\scriptstyle\face$}}
    \caption{The Boundary Representation (left) comprises several topological entities. Our Indexed Boundary Representation (right)  references vertices, edges, and faces in a well-defined hierarchy suitable for use with machine learning.}
    \label{fig:representation}
\end{figure*}
\myparagraph{Recovering a Boundary Representation.}
\label{ssec:recover_brep}
We leverage the boundary curve geometry that is defined by the edges $\edge$, together with the mapping of the edges that bound a face $\face$ to recover the wire and surface geometry using well-defined rules.
In particular, the surface type can be first fixed from the curve types while the surface parameters can be inferred from the curve and vertex geometry.
The surface type and parameters can be derived from the curves by a simple set of rules.  
For instance, faces whose vertices are coplanar define a trimmed planar surface, faces whose curves are a non-planar collection of lines and arcs will be cylinders or cones and faces whose curves are all arcs will be spheres or tori. 
We explain the procedure to apply this rule-based algorithm and build the B-rep in greater detail in  \autoref{sec:indexed_to_brep_conversion}.
Applying this procedure to every face in the indexed B-rep yields the surface type and parameters.
Then, the data is read into the solid modeling kernel using standard data exchange and shape fixing functions designed for reading neutral CAD file formats like STEP and IGES.

==> SolidGen TMLR arXiv/4-network.tex <==
\section{SolidGen Architecture}
SolidGen is a generative model that directly synthesizes CAD data in the B-rep format. 
SolidGen leverages Transformers~\citep{vaswani2017transformer} and pointer networks~\citep{vinyals2015pointer} to enable the generation of vertices, curved edges, and non-planar faces, such that edges can refer to vertices and faces can refer to edges, allowing us to build the complete B-rep topology.
Our goal is to estimate a distribution over indexed B-reps $\brep$ that can be sampled from to generate new indexed B-reps, and converted to actual B-reps as described in the previous section.
This probability distribution $p(\brep)$ is defined as the joint distribution of the vertices $\vertex$, edges $\edge$, and faces $\face$
\begin{equation}
p(\brep) = p(\vertex, \edge, \face).
\end{equation}
To make the learning problem tractable, we factorize this joint distribution into a product of conditionals
\begin{equation}
p(\brep) = p(\face|\edge,\vertex) p(\edge|\vertex)p(\vertex),
\label{eq:factorized}
\end{equation}
and learn these distributions with separate neural networks.
%%
Once these conditional distributions are learned, B-reps can be generated by sampling vertices first, followed by edges conditioned on vertices, and faces conditioned on the edges and vertices.
It is also possible to condition the generation using a context $z$ in which case the joint distribution becomes
\begin{equation}
p(\brep|z) = p(\face|\edge,\vertex,z) p(\edge|\vertex,z)p(\vertex|z),
\label{eq:factorized_conditioning}
\end{equation}
where $z$ can be derived from other representations like class labels, images, voxels, etc.
Since there can be an arbitrary number of vertices, edges, and faces in each B-rep, and strong symmetries are present in CAD models, we use autoregressive neural networks to model the probability distributions above. \autoref{fig:model} shows an overview of the SolidGen architecture at inference time, with each model described in further detail below.

\subsection{Vertex Model}
The vertex model (\autoref{fig:model}, left) learns a distribution $p(\vertex)$ over the vertex positions.
%%
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/SolidGenArchitecture-v03.pdf}
    \caption{The SolidGen architecture consists of a vertex (left), edge (center), and face (right) model that predict the vertices, edge connections between vertices, and face connections between edges to form an indexed B-rep (top).}
    \label{fig:model}
\end{figure*}
%%
Vertices here include both B-rep vertices and the additional points inserted on B-rep edges to encode the curve primitive information as explained in \autoref{ssec:recover_brep}.
The vertices are first sorted lexicographically, i.e., by z coordinates first, y coordinates next, and x coordinates finally, then their coordinates are flattened into a 1D list, with a stopping token \eostoken{} marking the end.
After flattening, $\vertexseq = \{v_0, v_1, \ldots, \eostoken{}\}$ is of length $\numvertexseq = (\numvertices \times 3) + 1$, with every triplet corresponding to coordinate values of a single vertex.
Rather than using real-valued coordinates for the vertices, we quantize the vertex sequence $\vertexseq$ uniformly into \numbits-bits as is common in previous work~\citep{nash2020polygen,seff2021vitruvion,wu2021deepcad}.
The vertex model learns the following distribution
\begin{equation}
p(\vertexseq; \thetav) = \prod_{t=0}^{\numvertexseq-1} p(v_t~|~v_0, v_1, \ldots, v_{t-1}; \thetav),
\end{equation}
where $\thetav$ are learnable parameters of the neural network that is a Transformer decoder~\citep{vaswani2017transformer}, and the conditional distributions above can all be treated as categorical distributions.

Given the input vertices $\vertexseqlt$ at step $t$, the goal is to model the next output vertex token $v_t$.
The input to the Transformer decoder $\hiddenvertex$ is derived from each of the tokens in $\vertexseqlt$ by learning three kinds of embeddings---\textit{coordinate embeddings} indicating whether a token is an x, y or z-coordinate, \textit{positional embeddings} indicating the vertex index which the token belongs to, and a \textit{value embedding} encoding the x, y or z-coordinate:
\[
\hiddenvertexseqlt = \{\embcoord(\onehot_{i \bmod 3}) + \embpos(\onehot_{\lfloor i \div 3 \rfloor} ) + \embval(\onehot_{v_i}) \}_{i=0}^{t - 1},
\]
where $\onehot$ maps its integer argument in the subscript into a one-hot vector, $\embcoord \in \mathbb{R}^{\demb \times 3}$, $\embpos \in \mathbb{R}^{\demb \times \numvertices}$ and $\embval \in \mathbb{R}^{\demb \times 2^\numbits}$ are all learned matrices that map their inputs to $\demb$=256 dimensional embeddings.
Then a Transformer decoder $\vertexdec$ model predicts a probability distribution (in the form of logits) over all possible vertex locations for the next token $v_t$:
\[
p(v_t) = \vertexdec(\hiddenvertexseqlt).
\]
The model is trained using teacher-forcing~\citep{williams1989teacherforcing} to maximize the log-likelihood of the training data with a cross-entropy loss with label smoothing of $0.01$.


\subsection{Edge Model}
The edge model (\autoref{fig:model}, center) learns a distribution $p(\edge)$ over the vertex indices.
The edges are represented as a 1D list $\edgeseq$ by flattening the vertex indices in $\edge$, with a new edge token \newedgetoken{} marking the start of a new edge and a stopping token \eostoken{} marking the end of the list.
For ordering invariance, we sort each edge $E \in \edge$ in ascending order and then sort $\edge$ such that the edges with lowest vertex indices come first.
The edge sequence $\edgeseq = \{e_0, e_1, \newedgetoken{}, \ldots, \eostoken{}\}$ is of length $\numedgeseq = \sum_{E\in \edge} |E| + 1$, and the edge model learns the following distribution:
%%
\begin{equation}
p(\edgeseq|\vertex; \thetae) = \prod_{j=0}^{\numedgeseq-1} p(e_j~|~e_0, e_1, \ldots, e_{j-1},\vertex; \thetae),
\end{equation}
%%
where $\theta_\edge$ are learnable parameters of the neural network.

Given the input vertices $\vertex$ and current edges $\edgeseqlt$ until the step $t$, the goal is to model the next output vertex index $e_t$ as a probability distribution over the indices of $\vertex$.
This is done by first learning \textit{value embeddings} $\hiddenvertex \in \mathbb{R}^{\numvertices \times \demb}$ from the input vertices $\vertex = \{ (x_i, y_i, z_i) \}_{i=0}^{\numvertices - 1}$:
\begin{equation}
\hiddenvertex = \left\{ \phi\left(\embx \onehot_{x_i} \concat \emby \onehot_{y_i} \concat \embz \onehot_{z_i}\right) \right\}_{i=0}^{\numvertices - 1},
\label{eq:embed_vertices}
\end{equation}
where $\embx$, $\emby$ and $\embz\in \mathbb{R}^{64\times 2^\numbits}$ are learned matrices that map their inputs into 64-dimensional embeddings, $\concat$ is the concatenation operation along the second dimension, and $\phi \in \mathbb{R}^{\demb \times (64\times 3)}$ is a learned linear layer to produce $\demb$=256 dimensional embeddings.
The token embeddings~ for $\newedgetoken{}$ and $\eostoken{}$, $\hiddennewedgetoken{} \in \mathbb{R}^{d_\text{emb}}$ and $\hiddeneostoken{} \in \mathbb{R}^{d_\text{emb}}$ are learnable parameters that are concatenated to form a total of $\numvertices+ 2$, which is further processed by Transformer encoder $\edgeenc$ to obtain $\hiddeninput \in \mathbb{R}^{(\demb \times \numvertices + 2)}$
\[
\hiddeninput     = \edgeenc(\hiddeneostoken \concat \hiddennewedgetoken \concat \hiddenvertex ).
\]
Then, edge embeddings $\hiddenedgeseqlt \in \mathbb{R}^{\numedgeseqlt \times 256}$ are formed by gathering the input embeddings $\hiddeninput$ corresponding to the vertex indices in $\edgeseqlt$ and summed with learned \textit{positional embeddings} indicating the position of each token in $\edgeseqlt$.
\[
\hiddenedgeseqlt = \{ \hiddeninput[e_j] + \embpos \onehot_j \}_{j=0}^{t-1},
\]
where $\embpos \in \mathbb{R}^{|\edgeseq|\times\demb}$ is a learnable matrix.

A Transformer decoder $\edgedec$ then processes these embeddings followed by a linear layer to output a pointer vector $\pointer_t$ that is compared to the input embeddings $\hiddeninput$ using a dot product operation and normalized using softmax to get a distribution over the $0 \le k \le \numvertices + 1$ indices including the vertex indices and the $\newedgetoken{}$, $\eostoken{}$ tokens:
\[
\begin{aligned}
\pointer_t       &= \edgedec(\hiddenedgeseqlt), \\
p(e_t = k~|~\edgeseqlt,\vertex) &= \softmax{k}(\pointer_t \cdot 
\hiddeninput[k]).
\end{aligned}
\]
The model is trained using the cross-entropy loss to predict the distribution $p(e_t = k~|~\edgeseqlt,\vertex)$ which is repeatedly created at each time step and sampled to generate the edge tokens autoregressively.
During training, ground-truth is used for conditioning (teacher-forcing) rather than previous samples.

\subsection{Face Model}
The face model (\autoref{fig:model}, right) learns a distribution $p(\face)$ over the faces.
The faces are represented as a flat sequence $\faceseq$ similar to the edges by flattening $\face$ into a 1D list of edge indices, with a new face token \newfacetoken{} marking the start of a new face and a stopping token \eostoken{} marking the end of the faces list.
The model learns the following probability distribution:
%%
\begin{equation}
p(\faceseq|\edge,\vertex; \thetaf) = \prod_{t=0}^{\numfaceseq-1} p(f_t~|~f_0, f_1, \ldots, f_{t-1}|\edge,\vertex; \thetaf),
\end{equation}
%%
where $\thetaf$ are learnable parameters of the neural network.

The face model functions similarly as the edge model and represents the face features by gathering edge embeddings.
Given the input vertices $\vertex$ and edges $\edge$, and the current faces $\faceseqlt$ at step $t$, the goal is to model the next output face token $f_t$ as a probability distribution over the indices of $\edge$.

This is done by learning vertex embeddings $\hiddenvertex' \in \mathbb{R}^{\numvertices\times \demb}$ from the input vertices as in \autoref{eq:embed_vertices}.
The rows of $\hiddenvertex'$ corresponding to the vertex indices in $\edge$ are first gathered and summed, and learned embeddings for \newfacetoken{} and \eostoken{}, $\hiddennewfacetoken{}$ and $\hiddeneostoken{}$ are further concatenated to these embeddings, and passed through a Transformer encoder $\edgeencinfacemodel$ to form $\hiddenedge \in \mathbb{R}^{(\numedges + 2) \times \demb}$:
\[
\hiddenedge = \edgeencinfacemodel(\{ \hiddeneostoken \concat \hiddennewfacetoken \concat \{\textstyle\sum_{v \in E} \hiddenvertex'[v]) \}_{E \in \edge} \}),
\]

Finally, face embeddings $\hiddenfaceseqlt$ are formed by gathering the edge embeddings which is further summed with learned \textit{positional embeddings}, and passed through another Transformer encoder $\faceenc$:
\[
\hiddenfaceseqlt = \faceenc(\{ \hiddenedge[f_k] + \embpos' \onehot_{k}\}_{k=0}^{t-1}),
\]
where $\embpos' \in \mathbb{R}^{|\faceseq|\times\demb}$ is a learnable matrix.
The idea here is to encode faces by the embeddings of the edges that lie on their boundary, and encode the edges by the embeddings of the incident vertices.

A Transformer decoder $\facedec$ then processes $\hiddenfaceseqlt$ to output a pointer vector $\pointer_t$ that is compared to the edge embeddings $\hiddenedge$ using a dot product operation and normalized using softmax to get a distribution over the $0 \le k \le \numedges + 1$ input edge indices and $\newfacetoken{}$, $\eostoken{}$ tokens: 
\[
\begin{aligned}
\pointer_t       &= \facedec(\hiddenfaceseqlt), \\
p(f_t = k~|~\faceseqlt,\edge,\vertex) &= \softmax{k}(\pointer_t \cdot 
\hiddenedge[k]).
\end{aligned}
\]
The face model is also trained by teacher-forcing using a cross-entropy loss.


==> SolidGen TMLR arXiv/5-experiments.tex <==
\section{Experiments}
In this section we perform experiments to qualitatively and quantitatively evaluate our method on unconditional generation, and various conditional generation tasks based on class labels, images, and voxels. 

\myparagraph{Implementation.~} Our implementation is in PyTorch~\citep{PyTorch}. 
We train our models for 1000 epochs with batch size 512 using the AdamW optimizer~\citep{loshchilov2019AdamW} (learning rate: 10$^{-4}$, weight decay: $0.01$) on an Nvidia DGX A100 machine.
The vertex, edge, and face models can be trained independently since we employ teacher-forcing where the models are decoupled during training---rather than using the samples from one model to condition the subsequent model, we use the ground truth data.
When a conditional embedding is jointly learned however, we have to train the three models together.
Training time ranges from 1--3 days depending on the dataset.
We find it critical for convergence to use the pre-LayerNorm variant of the Transformer~\citep{xiong2020prelayernorm}.
All Transformer modules use 8 layers with an embedding dimension of 256, and fully-connected dimension of 512 and 8 attention heads.
We initially experimented with 4, 8 and 12-layer models and observed the 8-layer model to work well. The 4-layer model was slightly underfitting while the 12-layer model was overfitting on our datasets.
To sample from the models we use nucleus  sampling~\citep{holtzman2020toppsampling}. We find it helpful to mask logits that are invalid in each step of the sampling (see \autoref{app:masking_logits}).
All data processing related to building indexed B-reps and reconstructing B-reps uses the OpenCascade/pythonOCC~\citep{pythonocc} solid modeling kernel.

\myparagraph{Datasets.~}
Publicly available datasets for B-rep solid models are limited compared to other 3D representations.
We demonstrate our method on two datasets while considering only files that contain the surface and curve types supported by the indexed B-rep format.\\
\textit{The Parametric Variations (PVar) Dataset}
is synthetically designed (see \autoref{app:pvar} for details) for testing SolidGen on the class-conditional generation task, since categorically labeled B-rep datasets are unavailable.
There are 120,000 models, 2000 in each of the 60 classes.
The dataset is split in a 90 (train)/5 (validation)/5 (test) proportion.\\
\textit{The DeepCAD Dataset}~\citep{wu2021deepcad}
contains a subset of the CAD models available in the ABC dataset~\citep{koch2019abc} that additionally includes the sequence of sketch and extrude CAD modeling operations. The original dataset contains 178,238 CAD models with a significant portion of duplicate and trivial models. We use a hash-based method, described in \autoref{sec:hashing}, to remove duplicates. We filter out trivial ($<8$ faces, for e.g., boxes), overly-complex ($>130$ faces) models, those that contain merged vertices after quantization and ones that yield very long  sequences with $>200$ tokens. We are left with 49,759 models that are split in 90/5/5 train/validation/test sets and used for all experiments.
For image conditioning, we render images of the CAD models with the OpenCascade viewer.
For voxel conditioning, we sample a point cloud with 2048 points from the surface of the CAD models, and quantize them into voxel grids of dimension $(2^\numbits)^3$ matching our vertex quantization.

\myparagraph{Metrics.}
\label{ssec:metrics}
We use the following metrics to quantitatively evaluate and compare SolidGen with other methods.
\textit{Valid} reports the percentage of solids that were successfully built and considered valid by the solid modeling kernel (see \autoref{app:valid_criteria}). \textit{Novel} measures the percentage of valid solids that are not duplicated from the training set, and \textit{Unique} reports the percentage of valid solids not duplicated within the sample set. The duplication check is based on our hashing procedure described in \autoref{sec:hashing}.

\subsection{Unconditional Generation}
\label{sec:uncond}
In this section we evaluate SolidGen on unconditional generation of B-reps.

\myparagraph{Modeling Performance.~} 
To evaluate the modeling performance, we report the negative log-likelihood (NLL) and per-step accuracy computed on the DeepCAD test set. The NLL is reported individually for our vertex, edge and face models in bits per vertex, bits per edge and bits per face, respectively. Since there is no other method that uses our indexed B-rep format, a one-to-one comparison is not possible and we use a `Uniform' model that allocates uniform probability to the entire co-domain of the data as a baseline reference. The accuracy corresponds to the top-$1$ prediction correctness of the next token given the ground truth for the previous tokens.
%%
\begin{table}
    \centering
    \caption{Modeling metrics for unconditional and conditional SolidGen models computed on the test set.}
    \small
    \begin{tabular}{llrrrrrrrr}
        \toprule
        \multirow{2}{*}{Dataset} & \multirow{2}{*}{Model} & \multicolumn{4}{c}{NLL (bits per, $\downarrow$)} &  \multicolumn{4}{c}{Top-$1$ Accuracy (\%, $\uparrow$)}\\
        \cmidrule(lr){3-6}\cmidrule(lr){7-10}
        & & Vert. & Edge & Face & Total & Vert. & Edge & Face & Mean\\
        \midrule
        \multirow{3}{*}{PVar}       & Uniform        & 18.44 & 13.59 & 24.96 & 56.99  &  2.01 &  1.59 &  2.04 & 1.88\\
                                    & SolidGen       & 4.49  & 0.01  & 0.04  & 4.54   & 91.30 & 99.97 & 99.88 & 97.05\\
                                    & w/class (vertex)& 4.19 & -     & -     & 4.24   & 83.20 & -     & -     & 94.35\\
                                    & w/class (all)   & 1.28 & 0.01  & 0.03  & 1.32   & 92.43 & 99.97 & 99.89 & 97.43\\
        \midrule
        \multirow{3}{*}{DeepCAD}    & Uniform         & 18.32 & 15.05& 28.14 & 61.51  & 1.48  & 1.10  & 1.42  & 1.33 \\
                                    & SolidGen        & 5.42  & 0.43 & 0.26  & 6.11   & 86.12 & 98.87 & 99.55 & 94.85\\
                                    & w/image (vertex) & 1.97 & -    & -     & 2.66   & 80.61 & -     & -     & 93.01\\
                                    & w/image (all)    & 1.98 & 0.26 &  0.27 & 2.51   & 89.74 & 98.84 & 99.31 & 95.96\\
                                    & w/voxel (vertex) & 4.89 & -    & -     & 5.42   & 82.28 & -     & -     & 93.48\\
                                    & w/voxel (all)    & 2.00 & 0.52 & 0.65  & 3.17   & 91.26 & 98.62 & 99.18 & 96.35\\
        \bottomrule
    \end{tabular}
    \label{tab:modeling_metrics}
\end{table}
%%
\autoref{tab:modeling_metrics} (first two rows under `DeepCAD') shows the quantitative metrics of our model and the uniform baseline on the DeepCAD~\citep{wu2021deepcad} dataset. 
SolidGen obtains an NLL of $4.54$ bits and $97.05\%$ accuracy compared to the `Uniform' model that has an NLL of $56.99$ bits and $1.88\%$ accuracy.
We find that the edge and face models always outperform the vertex model. This could be because once the vertices are estimated, the edges and faces are significantly constrained in our representation. We show plots for top-$10$ accuracy in \autoref{app:additional_results}.

\myparagraph{Comparison with DeepCAD.~}
We evaluate the quality of the generated samples produced by SolidGen and compare them with that of DeepCAD~\citep{wu2021deepcad} model.
Note that both models work in fundamentally different ways---SolidGen is an autoregressive generative model trained directly on the B-reps, while DeepCAD is an autoencoder that learns from sequences of CAD modeling operations. This fundamental difference in representation leads to differences in design choices making a fair comparison challenging. We strive to provide a one-to-one comparison by focusing mainly on the sample quality.
%%
\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/DeepCADDataset.jpg}
    \caption{Dataset}
    \label{fig:uncond_gt}
    \end{subfigure}
    \rulesep
    \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/DeepCADDeepCAD.jpg}
    \caption{DeepCAD}
    \label{fig:uncond_deepcad}
    \end{subfigure}
    \rulesep
    \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/DeepCADSolidGen.jpg}
    \caption{SolidGen (ours)}
    \label{fig:uncond_solidgen}
    \end{subfigure}
    \caption{Qualitative results for unconditional generation. Samples (a) from the DeepCAD dataset, (b) generated by the DeepCAD model~\citep{wu2021deepcad}, and (c) generated by SolidGen.}
    \label{fig:uncond}
\end{figure*}
%%
\autoref{fig:uncond} shows qualitative results for unconditional generation trained on the DeepCAD dataset~\cite{wu2021deepcad}. We show samples from the dataset for comparison (a), along with generated samples from DeepCAD (b) and SolidGen (c). More results are shown in \autoref{app:additional_results}.
%%
\begin{table}
    \centering
    \caption{Quality of 5000 unconditional samples generated by networks trained on the DeepCAD dataset. SolidGen results are shown for samples generated with different top-$p$ values in nucleus sampling.}
    \small
    \begin{tabular}{lcccc}
        \toprule
        Model 
        & {Valid (\%,$\uparrow$)}
        & {Novel (\%,$\uparrow$)}
        & {Unique (\%,$\uparrow$)}\\
        \midrule
        SolidGen (p=0.5) & 87.57 & 66.22 & 33.69 \\
        SolidGen (p=0.6) & 88.12 & 73.00 & 61.42 \\
        SolidGen (p=0.7) & 86.70 & 82.46 & 83.91 \\
        SolidGen (p=0.8) & 85.21 & 88.09 & 93.65 \\
        SolidGen (p=0.9) & 83.10 & 92.38 & 97.49\\
        \midrule
        DeepCAD          & 62.11  & 96.73 & 99.01 \\
        \bottomrule
    \end{tabular}
    \label{tab:uncond}
\end{table}
We present quantitative metrics in \autoref{tab:uncond}. A large portion of the models produced by SolidGen are valid and usable B-reps, with SolidGen showing between $20.99\%$ to $26.01$\% improvement in the valid ratio compared to DeepCAD.
By varying the top-$p$ hyperparameter in nucleus sampling, SolidGen is able to trade-off between validity and novelty and uniqueness of B-reps produced. We observe a clear trend where increasing $p$ reduces validity while increasing the novelty and uniqueness.
SolidGen falls slightly below DeepCAD and obtains $4.38\%$ to $30.51\%$ lower novel  and $1.52\%$ to $65.32\%$ lower unique ratio depending on the top-$p$ parameter.
We found that many of DeepCAD's samples contain self-intersections and tend to be noisy/unrealistic leading to decreasing the valid score, but artificially increasing the unique and novel scores. We further investigate this through a human perceptual study next.

\myparagraph{Human Perceptual Evaluation.}
%%
\begin{figure}
    \centering
    \includegraphics[width=0.95\columnwidth]{figures/UserStudy.pdf}
    \caption{Human perceptual study showing the distribution of votes by 7 human evaluators for the realism of SolidGen and DeepCAD models compared to samples from the training set.}
    \label{fig:human_eval}
\end{figure}
%%
Rather than rely only on metrics, we believe it is critical to perform human evaluation on the output of generative models.
To evaluate the realism of the generated samples, we perform a perceptual study using human evaluators recruited through Amazon's Mechanical Turk service \citep{mishra_2019}.
The crowd workers were shown pairs of images, one of which was generated by SolidGen ($p=0.7$) or DeepCAD and the other randomly selected from the training set, and asked to judge which of the two was more realistic.
Each image pair was rated by 7 different human evaluators and we record the number of crowd workers who selected the generated model as more realistic.  The results are shown in \autoref{fig:human_eval}. We see that for SolidGen the distribution is roughly symmetric with the majority vote judging the SolidGen output to be more realistic 52.67\% of the time.   This indicates the realism of the SolidGen output is indistinguishable from the training set.  For DeepCAD we see the distribution is skewed to the left, with the majority vote judging the DeepCAD output to be more realistic only 35.22\% of the time.

\myparagraph{Statistics.}
%%
\begin{figure}
    \centering
    \newcommand{\imgwidth}{0.18\columnwidth}
    %%
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/Densities/Num_vertices.pdf}
    \end{subfigure}
    %%
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/Densities/Num_edges.pdf}
    \end{subfigure}
    %%
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/Densities/Num_faces.pdf}
    \end{subfigure}
    %%
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/Densities/Num_line.pdf}
    \end{subfigure}
    %%
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/Densities/Num_arc.pdf}
    \end{subfigure}\\
    %%
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/Densities/Num_plane.pdf}
    \end{subfigure}
    %%
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/Densities/Num_cylinder.pdf}
    \end{subfigure}
    %%
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/Densities/Edge_length.pdf}
    \end{subfigure}
    %%
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/Densities/Face_area.pdf}
    \end{subfigure}
    %%
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/Densities/Volume.pdf}
    \end{subfigure}
    %%
    \caption{Comparison of distributions computed from SolidGen samples and the DeepCAD training set.}
    \label{fig:statistics}
\end{figure}
%%
To check if SolidGen synthesizes B-reps representative of the dataset, we compute several statistics between the samples produced by SolidGen (with top-$p$=$0.9$) compared to the DeepCAD training set in \autoref{fig:statistics}.
Here we used kernel density estimation with Gaussian kernels to fit the curves, and see that SolidGen well captures the modes of the data distribution.


\subsection{Conditional Generation}
\label{sec:cond}
In this section, we demonstrate various conditional generation results using class labels in the PVar dataset and rendered images and voxels from the DeepCAD dataset.
Conditional models use the same architecture, hyperparameters and training strategy as the unconditional model, and support two kinds of conditioning:\\
\textit{Start-of-sequence (SOS) Embedding.~} For class conditioning, we learn a $\demb$=$256$ dimensional embedding from the input class label, and use it as the SOS embedding in the vertex, edge and face models.\\
\textit{Cross Attention.~} For image/voxel conditioning, we use a 2D/3D convolutional neural network (details in \autoref{app:cnn}) to obtain an $16^2$/$8^3$ dimensional embedding that is flattened and jointly used by the Transformer decoders in the vertex, edge and face models via cross-attention.

\begin{figure}[t]
    \centering
    \newcommand\imgwidth{0.09\columnwidth}
    %%%
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/13_0.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/13_14.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/13_16.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/13_28.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/13_8.jpg}
    \end{subfigure}\rulesep
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/16_27.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/16_64.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/16_8.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/16_82.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/16_91.jpg}
    \end{subfigure}\\[-2ex]
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/22_13.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/22_2.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/22_24.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/22_32.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/22_6.jpg}
    \end{subfigure}\rulesep
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/29_0.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/29_1.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/29_2.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/29_4.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/29_8.jpg}
    \end{subfigure}\\[-2ex]
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/42_28.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/42_33.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/42_39.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/42_4.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/42_8.jpg}
    \end{subfigure}\rulesep
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/53_18.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/53_22.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/53_26.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/53_28.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ClsCond/53_4.jpg}
    \end{subfigure}%\\[-3ex]
    \caption{Class conditional samples (each row is a unique class) from SolidGen trained on the PVar dataset.
    }
    \label{fig:class_cond}
\end{figure}
%%
\begin{figure}
    \centering
    \newcommand\imgwidth{0.09\columnwidth}
    %%%
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth, trim=80 0 80 0, clip]{figures/ImgCond/00006190_img.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00006190_2.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00006190_5.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00006190_8.jpg}
    \end{subfigure}
    \begin{subfigure}[b]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00006190_10.jpg}
    \end{subfigure}\rulesep
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth, trim=80 0 80 0, clip]{figures/ImgCond/00031373_img.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00031373_4.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00031373_8.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00031373_14.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00031373_16.jpg}
    \end{subfigure}\\[-1ex]
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth, trim=80 0 80 0, clip]{figures/ImgCond/00078961_img.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00078961_0.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00078961_1.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00078961_2.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00078961_18.jpg}
    \end{subfigure}\rulesep
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth, trim=120 50 120 50, clip]{figures/ImgCond/00049639_img.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00049639_2.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00049639_4.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00049639_5.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00049639_8.jpg}
    \end{subfigure}\\[-1ex]
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth, trim=80 0 80 0, clip]{figures/ImgCond/00049317_img.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00049317_1.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00049317_10.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00049317_17.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00049317_2.jpg}
    \end{subfigure}\rulesep
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth, trim=80 0 80 0, clip]{figures/ImgCond/00009000_img.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00009000_0.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00009000_3.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00009000_5.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/ImgCond/00009000_9.jpg}
    \end{subfigure}
    \caption{Image conditional samples from SolidGen using images (first column) obtained by rendering CAD models in the DeepCAD test set. 
    }
    \label{fig:img_cond}
\end{figure}
%%
\begin{figure}
    \centering
    \newcommand\imgwidth{0.09\columnwidth}
    %%%
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00026350_vox.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00026350_1.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00026350_3.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00026350_5.jpg}
    \end{subfigure}
    \begin{subfigure}[b]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00026350_9.jpg}
    \end{subfigure}\rulesep
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00026773_vox.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00026773_1.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00026773_2.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00026773_6.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00026773_0.jpg}
    \end{subfigure}\\[-1ex]
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00035450_vox.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00035450_6.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00035450_7.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00035450_8.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00035450_9.jpg}
    \end{subfigure}\rulesep
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00079637_vox.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00079637_1.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00079637_4.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00079637_5.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00079637_9.jpg}
    \end{subfigure}\\[-1ex]
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00166713_vox.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00166713_0.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00166713_1.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00166713_4.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00166713_9.jpg}
    \end{subfigure}\rulesep
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00994797_vox.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00994797_7.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00994797_0.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00994797_2.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{\imgwidth}
    \includegraphics[width=\textwidth]{figures/VoxCond/00994797_5.jpg}
    \end{subfigure}
    \caption{Voxel conditional samples from SolidGen using voxelized point clouds (first column) obtained by sampling 2048 points from CAD models in the DeepCAD test set.}
    \label{fig:vox_cond}
\end{figure}
\myparagraph{Modeling Performance.~} The modeling performance of the conditional models are shown in Table~\ref{tab:modeling_metrics}. The `w/class (all)' row under `PVar' shows that class conditioning improves the NLL by $-3.22$ and accuracy by $+0.38\%$ compared to the unconditional `SolidGen' model trained on the same data.
A similar trend is observed for image and voxel conditioning shown under row `DeepCAD'. The NLL for the `w/image (all)' conditional model improved by $-3.6$ while the accuracy improved by $+3.6\%$. For the voxel conditional model `w/voxel (all)', the NLL improved by $-2.94$ while the accuracy increased by $+1.5\%$.

\myparagraph{Sample Quality.~} Qualitative results of our class-conditioning model given random class labels as input are shown in \autoref{fig:class_cond}. 
\autoref{fig:img_cond} shows B-reps produced by our model given images as input conditioning, while \autoref{fig:vox_cond} shows results where voxelized point clouds were used as conditioning. We see that SolidGen is able to synthesize design variations that are close to the input conditioning.
Quantitative evaluation of the class-conditional samples (40 per-class), image conditional samples (20 per image) and voxel conditional samples (20 per voxel grid) are provided in \autoref{tab:cond}.
We see that SolidGen generates a high number of novel B-reps, but the valid and unique ratio go down as we transition from class to image to voxel conditioning.  We suspect this trend is due to data imbalance in the dataset which contains arbitrary shapes without clear categories making the overall task challenging. Moreover, unlike unconditional and class conditional generation, image and voxel conditioning require generating design variations for every data in the test set, making the task more challenging. The less precise nature of 2D image conditioning makes it easier to learn and generate design variations compared to the 3D case.
%%
\begin{table}
    \centering
    \caption{Quality of conditional samples generated by SolidGen with top-$p$=0.7.}
    \small
    \begin{tabular}{lcccc}
        \toprule
        Conditioning 
        & {Valid (\%,$\uparrow$)}
        & {Novel (\%,$\uparrow$)}
        & {Unique (\%,$\uparrow$)}\\
        \midrule
        Class (PVar)     & 83.48 & 92.35 & 70.71 \\
        Image (DeepCAD) & 71.45 & 94.61 & 75.08\\
        Voxel (DeepCAD) &  66.78 & 92.75 & 53.95 \\
        \bottomrule
    \end{tabular}
    \label{tab:cond}
\end{table}

\myparagraph{Ablation on joint conditioning.} 
Conditional models require the vertex, edge and face models to be trained together. To understand the importance of jointly learning a conditional embedding for the vertex, edge and face models, we experimented with a variant of SolidGen where the conditioning is only applied to the vertex model. This variant denoted by `w/ \textasteriskcentered(vertex)' in \autoref{tab:modeling_metrics} has the advantage that the vertex, edge, and face models can be trained independently in parallel since the probability distribution being modeled is $p(\brep|z) = p(\face|\edge,\vertex) p(\edge|\vertex)p(\vertex|z)$. 
We observe that conditioning only the vertex model does improve the NLL in all cases (class:$-0.3$, image:$-3.45$, voxel:$-0.69$), but the accuracy drops below that of the unconditional model (class:$-2.7\%$, image:$-1.84\%$, voxel:$-1.37\%$). The joint conditioning variants `w/class (all)', `w/image (all)' and `w/voxel (all)' perform the best in all cases.

==> SolidGen TMLR arXiv/6-conclusion.tex <==
\section{Conclusion}
\myparagraph{Limitations \& Future Work.~}
Our current method has some limitations that can be addressed in future work.
Extremely complex CAD models with long sequence lengths increase the training time and chance for compounding errors at test time, which could be attributed to teacher forcing. Scaling our model and training on larger CAD datasets might alleviate the problem.
Our indexed B-rep format supports the most common curve and surface types found in mechanical CAD models but not conic sections and splines that are common in freeform modeling.
Uniform B-spline curves of a fixed degree can be supported by considering edges that group $>=(\text{degree}+1)$ vertices (the spline's control points). However, unlike prismatic surfaces, the B-spline surfaces cannot be fully determined by the boundary curves, and require the additional prediction of a grid of interpolating or control points.
Like previous generative neural networks~\citep{willis2021engineering,nash2020polygen,wu2021deepcad,xu2022skexgen} our method is trained using classification losses.
Several important CAD applications, e.g., reverse engineering, require reconstruction losses that incorporate the B-rep geometry which is not available until postprocess.
Finally, research into conditioning schemes could facilitate stronger user guidance in the generation, and latent representations would help with better generalization.

\myparagraph{Summary.~}
We presented SolidGen, a generative model that can directly learn from and synthesize boundary representation (B-rep) CAD models without the need for supervision from a sequence of CAD modeling operations.
We achieved this by deriving the indexed B-rep format that captures the hierarchical nature of B-rep vertices, edges and faces in a new machine learning friendly representation.
SolidGen generates highly coherent yet diverse B-reps as demonstrated in our comparison with prior work.
Our method has potential to be integrated into CAD software workflows, since all CAD software allows the import of solids without modeling history.
As our method can generate local regions of B-rep topology, in addition to entire solids, this allows learning-based techniques to play a role in many other workflows such as solid model inpainting and parting surface creation. Conditional generation can aid in sketch-based modeling workflows and to convert point clouds, meshes or other file formats into B-reps for further editing.

==> SolidGen TMLR arXiv/contents.tex <==
\input{notation}
\input{1-introduction}
\input{2-related-work}
\input{3-representation}
\input{4-network}
\input{5-experiments}
\input{6-conclusion}

==> SolidGen TMLR arXiv/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> SolidGen TMLR arXiv/notation.tex <==
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}

\newcommand{\vertex}{\mathcal{V}}
\newcommand{\edge}{\mathcal{E}}
\newcommand{\face}{\mathcal{F}}
\newcommand{\surface}{\mathcal{S}}
\newcommand{\brep}{\mathcal{B}}
\newcommand{\brepflat}{\brep_\text{flat}}
\newcommand{\indexedsolid}{Indexed Solid}
\newcommand{\vertexseq}{\vertex^\text{seq}}
\newcommand{\vertexseqlt}{\vertexseq_{<t}}
\newcommand{\edgeseq}{\edge^\text{seq}}
\newcommand{\edgeseqlt}{\edgeseq_{<t}}
\newcommand{\faceseq}{\face^\text{seq}}
\newcommand{\faceseqlt}{\faceseq_{<t}}
\newcommand{\eostoken}{\texttt{<EOS>}}
\newcommand{\sostoken}{\texttt{<SOS>}}
\newcommand{\newedgetoken}{\texttt{<NEW\_EDGE>}}
\newcommand{\newfacetoken}{\texttt{<NEW\_FACE>}}
\newcommand{\hiddenvertex}{\textbf{h}_\vertex}
\newcommand{\hiddenvertexseq}{\textbf{h}_\vertexseq}
\newcommand{\hiddenvertexseqlt}{\textbf{h}_{\vertexseqlt}}
\newcommand{\hiddenedge}{\textbf{h}_\edge}
\newcommand{\hiddenedgeseq}{\textbf{h}_{\edgeseq}}
\newcommand{\hiddenedgeseqlt}{\textbf{h}_{\edgeseqlt}}
\newcommand{\hiddenface}{\textbf{h}_\face}
\newcommand{\hiddenfaceseq}{\textbf{h}_{\faceseq}}
\newcommand{\hiddenfaceseqlt}{\textbf{h}_{\faceseqlt}}
\newcommand{\hiddeneostoken}{\textbf{h}_{\eostoken{}}}
\newcommand{\hiddennewedgetoken}{\textbf{h}_{\newedgetoken{}}}
\newcommand{\hiddennewfacetoken}{\textbf{h}_{\newfacetoken{}}}
\newcommand{\hiddeninput}{\textbf{h}_\text{inp}}
\newcommand{\hiddeninputedge}{\hiddeninput^\edge}
\newcommand{\hiddeninputface}{\hiddeninput^\face}
\newcommand{\pointer}{\mathbf{p}}
\newcommand{\edgeenc}{T^\edge_\text{enc}}
\newcommand{\edgedec}{T^\edge_\text{dec}}
\newcommand{\edgeencinfacemodel}{\bar{T}^\edge_\text{enc}}
\newcommand{\faceenc}{T^\face_\text{enc}}
\newcommand{\facedec}{T^\face_\text{dec}}
\newcommand{\vertexdec}{T^\vertex_\text{dec}}
\newcommand{\softmax}[1]{\text{softmax}_{#1}}
\newcommand{\numvertices}{|\vertex|}
\newcommand{\numvertexseq}{|\vertexseq|}
\newcommand{\numedges}{|\edge|}
\newcommand{\numedgeseq}{|\edgeseq|}
\newcommand{\numedgeseqlt}{|\edgeseqlt|}
\newcommand{\numfaces}{|\face|}
\newcommand{\numfaceseq}{|\faceseq|}
\newcommand{\thetav}{\theta_\vertex}
\newcommand{\thetae}{\theta_\edge}
\newcommand{\thetaf}{\theta_\face}
\newcommand{\concat}{\mathbin\Vert}
\newcommand{\numbits}{6}
\newcommand{\demb}{d_\text{emb}}
\newcommand{\embmatrix}{\mathbf{W}}
\newcommand{\embcoord}{\embmatrix_{\text{coo}}}
\newcommand{\embval}{\embmatrix_{\text{val}}}
\newcommand{\embpos}{\embmatrix_{\text{pos}}}
\newcommand{\embx}{\embmatrix_{\text{x}}}
\newcommand{\emby}{\embmatrix_{\text{y}}}
\newcommand{\embz}{\embmatrix_{\text{z}}}
\newcommand{\eosedge}{\texttt{EOE}}
\newcommand{\eoswire}{\texttt{EOW}}
\newcommand{\eosface}{\texttt{EOF}}
\newcommand{\onehot}{\mathbbm{1}}


\newcommand{\convtwo}[4]{\text{Conv2d}(#1,#2,#3,#4)}
\newcommand{\convthree}[4]{\text{Conv3d}(#1,#2,#3,#4)}
\newcommand{\gelu}{\text{GELU}()}
\newcommand{\dropout}[1]{\text{Dropout}(#1)}

==> SolidGen TMLR arXiv/preamble.tex <==
\usepackage{picture}
\usepackage{multirow}
\usepackage{enumitem}
\usepackage{soul}
\usepackage{amsmath}
%\usepackage{hyperref}
\usepackage{bbm}
\usepackage{subcaption}
\usepackage{pgffor}
\usepackage{amssymb}
\makeatother
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage[T1]{fontenc}

\newcommand{\papertitle}{SolidGen: An Autoregressive Model for Direct B-rep\\Synthesis}

\newcommand{\rulesep}{\unskip\ \vrule\ }
\def\sectionautorefname{Section}%
\def\subsectionautorefname{Section}%
\newcommand{\myparagraph}[1]{\noindent\textbf{#1}}


==> SolidGen TMLR arXiv/templates/tmlr/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> templates/tmlr/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

